Machine Learning for Combinatorial Optimization: a Methodological Tour d'Horizon

This paper surveys the recent attempts, both from the machine learning and operations research communities, at leveraging machine learning to solve combinatorial optimization problems. Given the hard nature of these problems, state-of-the-art algorithms rely on handcrafted heuristics for making decisions that are otherwise too expensive to compute or mathematically not well defined. Thus, machine learning looks like a natural candidate to make such decisions in a more principled and optimized way. We advocate for pushing further the integration of machine learning and combinatorial optimization and detail a methodology to do so. A main point of the paper is seeing generic optimization problems as data points and inquiring what is the relevant distribution of problems to use for learning on a given task.

==> glossary.tex <==
% High level fields
\newacronym{or}{OR}{operations research}
\newacronym{co}{CO}{combinatorial optimization}
\newacronym{ml}{ML}{machine learning}
\newacronym{dl}{DL}{deep learning}
\newacronym{rl}{RL}{reinforcement learning}

% Machine learning lingo
\newacronym{iid}{iid}{independent and identically distributed}
\newacronym{sgd}{SGD}{stochastic gradient descent}
\newacronym{mdp}{MDP}{markov decision process}

% Neural networks
\newacronym{nn}{NN}{neural network}
\newacronym{mlp}{MLP}{multilayer perceptron}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{rnn}{RNN}{recurrent neural network}
\newacronym{gnn}{GNN}{graph neural network}
\newacronym{gan}{GAN}{generative adversarial network}

% Optimization lingo
\newacronym{tsp}{TSP}{traveling salesman problem}
\newacronym{lp}{LP}{linear programming}
\newacronym{milp}{MILP}{mixed-integer linear programming}
\newacronym{qp}{QP}{quadratic programming}
\newacronym{miqp}{MIQP}{mixed-integer quadratic programming}
\newacronym{sdp}{SDP}{semidefinite programming}
\newacronym{bnb}{B\&B}{branch-and-bound}
\newacronym{sat}{SAT}{boolean satisfiability problem}

% Computer lingo
\newacronym{gpu}{GPU}{graphical processing unit}
